Scalable Factor Graph-Based Heterogeneous Bayesian DDF for Dynamic Systems

Heterogeneous Bayesian decentralized data fusion captures the set of problems in which two robots must combine two probability density functions over non-equal, but overlapping sets of random variables. In the context of multi-robot dynamic systems, this enables robots to take a "divide and conquer" approach to reason and share data over complementary tasks instead of over the full joint state space. For example, in a target tracking application, this allows robots to track different subsets of targets and share data on only common targets. This paper presents a framework by which robots can each use a local factor graph to represent relevant partitions of a complex global joint probability distribution, thus allowing them to avoid reasoning over the entirety of a more complex model and saving communication as well as computation costs. From a theoretical point of view, this paper makes contributions by casting the heterogeneous decentralized fusion problem in terms of a factor graph, analyzing the challenges that arise due to dynamic filtering, and then developing a new conservative filtering algorithm that ensures statistical correctness. From a practical point of view, we show how this framework can be used to represent different multi-robot applications and then test it with simulations and hardware experiments to validate and demonstrate its statistical conservativeness, applicability, and robustness to real-world challenges.

==> Text/3_DDF.tex <==
Given two agents i and j, we are interested in forming an estimate of the state $\chi$ given all the information available locally, defined by $Z^i$ and $Z^j$, respectively. Assuming all measurements are conditionally independent given the state $\chi$ and using a distributed variant of Bayes' rule, \cite{chong_distributed_1983} shows that the exact state estimate can be achieved using:
\begin{equation}
    p_f(\chi|Z^{i,-}_k\cup Z^{j,-}_k)\propto \frac{p^i(\chi|Z^{i,-}_k)p^j(\chi|Z^{j,-}_k)}{p^{ij}_c(\chi|Z^{i,-}_k\cap Z^{j,-}_k)}
    \label{eq:Homogeneous_fusion}
\end{equation}
where $p^{ij}_c(\chi|Z^{i,-}_k\cap Z^{j,-}_k)$ is the distribution of the common information (when it makes sense to define one) of the two agents which needs to be removed in order to avoid double counting. Notice that the above fusion rule satisfies  (\ref{eq:probStatement}) for the homogeneous case $\chi=\chi^i=\chi^j$. \\
In this paper we assume that common information is explicitly tracked, by either keeping a pedigree of all information transformed in fusion instances or by restricting network topology to a tree structure, as in the channel filter \cite{grime_data_1994}.

For heterogeneous fusion, $\chi^i\neq \chi^j$, assuming the local states are conditionally independent given common states:
\begin{equation*}
    \chi^i_L\perp \chi^j_L \mid \chi^{ij}_C,
\end{equation*}
Dagan \textit{et al.} show in \cite{dagan_exact_2021} that agents can fuse only a subset of common variables without the need to communicate ``irrelevant" local variables. The fusion rule at agent $i$ can be written as,
\begin{equation}
    \begin{split}
        p^i_f(\chi^i|Z^{i,+}_k)\propto
        \frac{p^i(\chi^{ij}_C|Z^{i,-}_k)p^j(\chi^{ij}_C|Z^{j,-}_k)}{p^{ij}_c(\chi^{ij}_C|Z^{i,-}_k\cap Z^{j,-}_k)}\cdot p^i(\chi^i_L|\chi^{ij}_C,Z^{i,-}_k).
    \end{split}
    \label{eq:Heterogeneous_fusion}
\end{equation}
In \cite{dagan_exact_2021}, assuming tree topology, this is named the \emph{heterogeneous-state channel filter} (HS-CF).
As we show later, (\ref{eq:Heterogeneous_fusion}) amounts to sending/incorporating a factor in the local graph of each of the agents $i/j$.

We move our attention to factor graphs, we describe and define them for general pdfs and for the special case of Gaussian distributions (Sec. \ref{sec:FactorGraphs}). We then put it all together in Sec. \ref{sec:FG_DDF} to formalize factor graphs for DDF.   

==> Text/4_Factor_graphs.tex <==
\begin{figure}[b]
	\centering
	\includegraphics[width=0.52\textwidth]{Figures/factor_graph_fig2.pdf}
	\caption{a) Example factor graph representing a tracking scenario, where the variables of interest are the target states from time $t=0$ to $t=k$. Shown are the different types of factors (prior, transition and measurement). b-d) show the graph operations, namely prediction, roll-up and estimation, with new factors and variables marked by red empty nodes.  } 
	\label{fig:factorGraph_operations}
	\vspace{-0.1in}
\end{figure}

A factor graph is an undirected bipartite graph $\mathcal{F}=(U,V,E)$ with factor nodes $f_l\in U$, random variable nodes $v_m\in V$ and edges $e_{lm}\in E$ connecting factor node \emph{l} to variable node \emph{m}. Each factor $f_l$ has one set of neighboring variable nodes $V_l\in V$ such that $f_l(V_l)$ is a function of only those variables in $V_l$. The joint distribution over the graph is then proportional to the global function $f(V)$, factorized by $f_l(V_l)$:
\begin{equation}
    p(V)\propto f(V)=\prod_{l}f_l(V_l)
    \label{eq:factorization}
\end{equation}

For a more complete description of factor graphs and algorithms for different operations on the graphs see \cite{frey_factor_1997}. For factor graphs in the context of robotics and graph-SLAM see \cite{dellaert_factor_2017}.



\begin{comment}


\begin{figure}[tb]
      \centering
      %\framebox{\parbox{3in}{}
      \missingfigure[figwidth=6cm]{Put an example factor graph here}
      \caption{}
      \label{fig:factorGraph}
      %\vspace{-0.2in}
\end{figure}
\end{comment}
An example of a factor graph describing a simple tracking problem, where the variables $v_m$ describe the target position states in time $x_k$, can be seen in Fig. \ref{fig:factorGraph_operations}a. Here 
we have three types of factors: a prior, a measurement likelihood and a dynamic transition factors. The posterior distribution, given the measurements, is then proportional to the factorization of the global function:
\begin{equation}
    \begin{split}
        p(x_{k:0}|y_{k:1})\propto f(x_0)\prod_{k=1}^{K}f(x_k;y_k)f(x_k|x_{k-1}),
    \end{split}
\end{equation}
where we use $f(x_k|x_{k-1})=f(x_k,x_{k-1})\propto p(x_k|x_{k-1})$ and $f(x_k;y_k)=f(x_k)\propto l(x_k;y_k)$ to express and emphasize conditional probabilities between variables and between variables to measurements, respectively. This is based on the idea in \cite{frey_extending_2002} of extending factor graphs to represent directed (Bayesian networks) and undirected (Markov random fields), thus making dependencies explicit when reading the factor graph.\\   
As we show in more detail later, in DDF, fusion is done by incorporating a new factor into the local graph, representing the new information that agent $i$ received from agent $j$. 

\subsection{Factor Graphs in Gaussian Canonical Form}
A factor graph $F=(U,V,E)$ represents the distribution $p(V)$ by a product of its factors (see (\ref{eq:factorization})). This can be transformed to a summation by converting the factors to log-space as described in \cite{koller_probabilistic_2009}. A special case is the canonical (information) form of linear Gaussian distributions; factors then consists of two elements, namely the information vector and matrix, that in turn can be summed over the graph to describe the multivariate Gaussian distribution in canonical form,
\begin{equation}
    p(V)\sim \mathcal{N}(\zeta, \Lambda)= \sum_{l}f_l(V_l).
    \label{eq:canonicalFactorization}
\end{equation}
Here $\zeta$ and $\Lambda$ are the information vector and matrix, respectively. In this case all factors are Gaussian distributions represented in canonical form $f_l(V_l)\sim \mathcal{N}(\zeta_l, \Lambda_l)$.

\subsection{Probabilistic Operations on Factor Graphs}
In \cite{paskin_thin_2002} a graphical model perspective of the SLAM problem is discussed. In order to reduce the size of the graph a filtering approach is taken by defining three types of operations on the dynamic Bayes net (DBN) type graph. The three operations are: \emph{prediction}, \emph{roll-up} (marginalization of past states) and \emph{estimation} (measurement update). We follow \cite{paskin_thin_2002} and the information augmented state (\emph{iAS}) filter presented in \cite{dagan_exact_2021} to define these operations on a factor graph and show their translation into new factors.\\
\emph{Prediction:}\\
In the prediction step three factors are added to the graph: two unary factors $f^-(x_k), f^-(x_{k+1})$, connected to the variable nodes $x_k$ and $x_{k+1}$, respectively, and a binary factor $f^-(x_{k+1}|x_k)$ connected to both variables and describes the correlation between the two variables. The $(-)$ superscript denotes prediction. Each factor is defined by an information vector and matrix $\{\zeta, \Lambda\}$:
\begin{equation}
    \begin{split}
        f^-(x_k) &= \{-F_k^TQ_k^{-1}G_ku_k,\ F_k^TQ_k^{-1}F_k\} \\
        f^-(x_{k+1}) &= \{Q_k^{-1}G_ku_k, \ Q_k^{-1} \} \\ 
        f^-(x_{k+1}|x_k) &= \left \{ \begin{pmatrix}
        0_{n\times1} \\ 0_{n\times1}
        \end{pmatrix}, \begin{pmatrix}
        0_{n\times n} & -Q_k^{-1}F_k\\ 
        -F_k^TQ_k^{-1} & 0_{n\times n}
        \end{pmatrix} \right \}.
    \end{split}
    \label{eq:predFactors}
\end{equation}
Here $F_k$ and $G_k$ are the state transition and control matrices at time step $k$, respectively. $u_k$ is the input vector and $Q_k$ is a zero mean white Gaussian process noise covariance matrix. The graphical description of the prediction step is given in Fig. \ref{fig:factorGraph_operations}b.\\
\emph{Roll-up (marginalization):}\\
It is known that upon marginalization of a random variable $x$ in a directed graphical model, all variables in the Markov blanket of $x$ are moralized, i.e. ``married'' by adding an edge. The effect in a factor graph is similar, and variables are moralized by adding a factor connecting all variables in the Markov blanket of the marginalized variable. If we denote the Markov blanket of $x$ by $\bar{x}$, then the new factor $f(\bar{x})$ is computed in two steps:\\
1. Sum all factors connected to $x$ to compute the following information vector and matrix:
\begin{equation}
    \{\zeta,\ \Lambda \} = f(x)+\sum_{i\in \bar{x}}f(x,\bar{x}_i)
\end{equation}
2. Use Schur complement to compute the marginal and find the new factor $f(\bar{x})$:
\begin{equation}
    f(\bar{x}) = \{\zeta_{\bar{x}}-\Lambda_{\bar{x}x}\Lambda_{xx}^{-1}\zeta_x,\  \Lambda_{\bar{x}\bar{x}}-\Lambda_{\bar{x}x}\Lambda_{xx}^{-1}\Lambda_{x\bar{x}}\}.
    \label{eq:marginalFactor}
\end{equation}
Notice that as a result, conditionally independent variables become correlated.\\
We demonstrate marginalization in Fig. \ref{fig:factorGraph_operations}c, marginalizing out $x_{k:n}$ induces a new factor $f(x_{k+1})$ over $x_{k+1}$. Here, since the only variable in the Markov blanket of the marginalized variables is $\bar{x}=x_{k+1}$, the new factor is unary over $x_{k+1}$ alone.\\
\emph{Estimation (measurement update):}\\
Adding a measurement in the canonical (information) form of the Kalman filter is a simple task. In the factor graph this translates to adding a factor $f(x_{k+1};y_{k+1})$ connected to all measured variables,
\begin{equation}
    f(x_{k+1};y_{k+1}) = \{H_{k+1}^TR_{k+1}^{-1}y_{k+1},\ H_{k+1}^TR_{k+1}^{-1}H_{k+1} \}.
    \label{eq:measFactors}
\end{equation}
Where $H_{k+1}$ is the sensing matrix, $R_{k+1}$ is a zero mean white Gaussian measurement noise covariance matrix and $y_{k+1}$ is the noisy measurement vector.
Figure \ref{fig:factorGraph_operations}d shows the addition of a unary measurement factor $f(x_{k+1};y_{k+1})$.
\begin{comment}


\begin{figure}[tb]
      \centering
      %\framebox{\parbox{3in}{}
      \missingfigure[figwidth=6cm]{Put an example of the graph operations here}
      \caption{}
      \label{fig:factorGraph_operations}
      %\vspace{-0.2in}
\end{figure}
\end{comment}






==> Text/Conditional_CF.tex <==
\begin{comment}
Let $p(\chi|Z_k)$ be the posterior distribution of the state $\chi$, an $n$-dimensional vector of random variables given all data received up to time $k$. Assume $\chi$ is tracked by a network of $N_a$ autonomous agents performing recursive decentralized Bayesian estimation. Each agent $i\in \{1,...,N_a\}$ has two sources of information $Z_{i,k}$: i) independent sensor data $Y_{i,k}$ described by conditional likelihood $p(Y_{i,k}|\chi)$ and ii) external information previously received from any other agent $j\in \{1,...,N_a, i\neq j\}$ in the network and fused by $i$. The posterior distribution is found by the respective separate updates of the prior distribution $p_i(\chi|Z_{i,k-1})$: first,  measurement update that can be updated locally by
\begin{equation}
    p_i(\chi|Z^{-}_{i,k})\propto p_i(\chi|Z_{i,k-1})\cdot p(Y_{i,k}|\chi)
    \label{eq:measUpdate}
\end{equation}
where $p_i(\chi|Z_{i,0})=p_0(\chi)$ is the common prior distribution. Second, fusion of new information received from all agents $j\in N_{i,k}$ communicating with agent $i$ at time step $k$ is represented by the following posterior fusion pdf,
\begin{equation}
    p_i(\chi|Z^{+}_{i,k})= p_i(\chi|Z^{-}_{i,k}\bigcup_{j\in N_{i,k}} Z^{-}_{j,k})
    \label{eq:generalFusion}
\end{equation}
\noindent For homogeneous fusion, this pdf can be constructed by using different exact or approximate fusion rules, as discussed previously. However, we are interested in heterogeneous fusion problems, i.e. where either: i) two agents $i$ and $j$ maintain local posterior pdf distributions, $p_i(\chi_{i}|Z_{i,k})$ and $p_j(\chi_{j}|Z_{j,k})$, of two \emph{heterogeneous} (unequal) but overlapping state vectors $\chi_i$ and $\chi_j$, respectively, or ii) the communicated pdfs are over heterogeneous joint distributions, in other words, when the information in $Z^{-}_{i,k}$ and $Z^{-}_{j,k}$ ($i\neq j)$ is over a different set of overlapping states.

While the local measurement update given in (\ref{eq:measUpdate}) can be performed without change, the existing fusion rules for homogeneous distributions cannot be used and a new fusion rule to describe (\ref{eq:generalFusion}) is needed. 
We seek a new posterior pdf fusion rule, which can be defined generally by
\begin{equation}
        (p_i(\chi_i|Z_{i,k}^{+}), p_j(\chi_j|Z^{+}_{j,k})) = \mathbb{F}(p_i(\chi_i|Z^{-}_{i,k}), p_j(\chi_j|Z^{-}_{j,k})).
    \label{eq:probStatement}
\end{equation}
Here, the updated pdfs after fusion may not be equal, $p_i(\chi_i|Z^{+}_{i,k})\neq  p_j(\chi_j|Z^{+}_{j,k})$, especially in the case of fusion with respect to heterogeneous random state vectors.

Current homogeneous methods directly account for dependencies between monitored states, but do not give a solution to indirect dependencies between states not mutually monitored by both agents, as in the case of heterogeneous distributions. Mishandling these dependencies might lead to double-counting of common information and inconsistencies, e.g. such that (for MMSE estimation) locally estimated MSEs are too optimistic for local states. Thus, a function $\mathbb{F}$ that properly accounts for hidden dependencies is needed. 
\end{comment}

\begin{comment}


\subsection{Related Work}
\label{sec:realatedWork}
The idea of splitting a global state vector into $N$ subsets of $N_a$ vectors ($N_a \ll N$) has been posed to solve two different problems. The first problem, as presented for example in \cite{chen_fusion_nodate, noack_fusion_2014, klemets_hierarchical_2018, radtke_distributed_nodate}, tries to reconstruct an \emph{MMSE estimate} of the global state vector, by fusing $N_a$ local heterogeneous \emph{estimates}. The second problem, which is the focus of this paper, \emph{tries to find $N_a$ different local posterior pdfs}, given all the information locally available up to current time.

The problem of locally fusing information from a non-equal state vector dates back to \cite{berg_model_1991}. While that work offers a simple way for distributing into heterogeneous local state vectors, it assumes that the local pdfs are decoupled. In \cite{khan_distributed_nodate}, Khan et al. relax that assumption, but ignore dependencies between states in the fusion step and restricts the state distribution to only  states that are directly sensed by local sensors, where in practice, an agent might be ``interested" in a larger set of local states that are not all directly sensed. In \cite{chong_graphical_2004}, Chong et al. use conditional independence in Bayesian networks to reduce the subset of states to be communicated. However, they only use the conditional independence of measurements given system states, and do not utilize the conditional independence of subsets of states given other states, as considered here. The work by Whitacre et al. \cite{whitacre_decentralized_2011}, does not formally discuss conditional independence but introduce the idea of marginalizing over common states to fuse Gaussian distributions, when cross correlations of common states are known. However, they implicitly assume cross correlations among the conditioned, or unique, states are small. While this assumption might hold for the application therein, it does not offer a robust solution. Ref. \cite{ahmed_factorized_2016} use CI with Gaussian distributions to relax the assumption of known correlations of the fused state. 
Ref.\cite{saini_decentralized_nodate-1} suggests a similar solution to ref. \cite{ahmed_factorized_2016} but restrict it to systems where all agents have the same set of common states.
Although scalable and simple, such approaches do not account for dependencies between locally exclusive states. 

These dependencies are key to the problem, since they lead to coupled uncertainties and correlated estimation errors. For example, consider a simple target tracking problem with one target and two tracking agents. Assume the agents have perfect ownship position information, but unknown constant biases $s_i$ and $s_j$ in the agent-target relative measurement vectors $y_{i,k}$ and $y_{j,k}$, respectively. The agents can also take relative observations $m_{i,k}$ and $m_{j,k}$ to different landmarks to locally estimate these ownship measurement biases. As shown in Fig. \ref{fig:GraphModel}, two agents $i$ and $j$ become coupled due to the common target measurements. In the homogeneous case, the two agents process and communicate each other's ownship bias states in addition to the target states and explicitly account for their dependencies. But in the heterogeneous case, each agent is assumed to only estimate target states and its local own biases. The question is how to account for these dependencies during fusion, when these are not explicitly present in the local posterior pdfs.

This work aims to gain insight and understanding on how such issues should be addressed. By exploiting both the conditional independence structure of such problems, as can be seen from the graphical model in Fig. \ref{fig:GraphModel}, and the observability characteristics of the underlying dynamical system. We next show how to extend the channel filter (CF) fusion algorithm to a new family of exact and approximate \emph{conditionally factorized CF} methods for heterogeneous fusion. 
\end{comment}

\begin{figure}[tb]
      \centering
      %\framebox{\parbox{3in}{}
      \includegraphics[scale=0.4]{Figures/GraphModel2_v2.eps}
      \caption{(a) Static and (b) Partially dynamic Bayesian networks for two local random vectors $s_i/s_j$ (ownship measurement biases) and one common random vector $x$ (target state). In (a), the static state $x$ d-separates $s_i$ and $s_j$; in (b)   $x_{1:k}$ is required for d-separation. \od{I need to reference Makarenko \cite{makarenko_decentralised_2009} somewhere, also: \cite{bailey_decentralised_2007,bailey_decentralised_2011}}}
      \label{fig:GraphModel}
      \vspace{-0.2in}
\end{figure}

  

%%%%%%%%%%%%%%% old statement:
\begin{comment}
Given two agents \emph{i} and \emph{j} local measurements, we are interested to find the MMSE estimates of all targets tracked by the two agents and their ownship states, while the state vectors $\pmb{\chi}_k^i$ and $\pmb{\chi}_k^j$ are generally unequal, but has at least one state in common.\\
Hence, the definition of fusion between \emph{i} and \emph{j} is  the construction of the following MMSE estimates:
\begin{equation}
    \begin{split}
        (\pmb{\hat{\chi}}_k^{i+}, \hat{\Sigma}_k^{\pmb{\chi}^i+}, \pmb{\hat{\chi}}_k^{j+}, \hat{\Sigma}_k^{\pmb{\chi}^j+}) =\\ \mathbb{F}(\pmb{\hat{\chi}}_k^{i-}, \hat{\Sigma}_k^{\pmb{\chi}^i-},\ \pmb{\hat{\chi}}_k^{j-}, \hat{\Sigma}_k^{\pmb{\chi}^j-}) \nonumber
    \label{eq:probStatement}
    \end{split}
\end{equation}

\end{comment}
Our approach assumes a tree structured network and starts with a general probabilistic CF formulation. Then, as seen in Fig. \ref{fig:fusionChart}, we enumerate different fusion problems of interest. 
Starting from the original homogeneous CF (where all agents keep an estimate of the full global joint pdf), we then consider cases where an agent is only interested in and/or observes a subset of the global joint distribution. It is shown that by leveraging conditional independence, we can communicate only marginal state information, leading to the \emph{factorized CF (F-CF)} and the \emph{"Bi-directional" factorized CF (BDF-CF)}, depending on whether marginal information is sent in one or two directions, respectively. These extensions to the CF enable communication reduction by sending only new and relevant information while maintaining the accuracy of the original CF.

A branch of approximate CF methods include the \emph{approximate BDF-CF} and the \emph{heterogeneous state CF (HS-CF)}. In these we communicate only marginal information over common subsets, leaving the information over the unique subset of variables local at each agent. The main difference between these two methods is the size of the local joint distributions which influences the local processing requirements. In approximate BDF-CF, each agent processes its unobserved variables in order to get a rough estimate over less relevant states, for example. However, in HS-CF, the local joint distribution is minimized to hold only locally relevant variables, which significantly reduces computation.  

\begin{figure}[b]
	\centering
	\includegraphics[width=0.48\textwidth]{Figures/fusion_chart_noWEP_v4.eps}
	\caption{Different CFs derived in this paper, %with different levels of assumptions and approximations are described, 
	where the first three blocks describe exact fusion and the dashed blocks approximate, with %In the blocks we see the local state vectors and the subsets to be fused. We distinguish between 
	local relevant states $s=[s_i^T, s_j^T]^T$ and common states of interest $x$ for fusion shown. }
	\label{fig:fusionChart}
\end{figure}

\subsection{Preliminaries}
We define the full state $\chi$,  in the following way
\begin{equation}
    \chi=\begin{bmatrix}
    x\\
    s\\
    \end{bmatrix} \ \ \ \in\mathbb{R}^{(n_x+n_s)\times1}  \\
    \label{eq:stateDef}
\end{equation}
where $x$ and $s$ can generally describe vectors with $n_x$ and $n_s$ elements, respectively, for example: $x=[x_1,x_2,...,x_{n_x}]^T$.  
The state vector $\chi$ can be described by the multivariate joint probability density function (pdf), $p(\chi)=p(x,s)$. 
\subsubsection{Factorization}
From the law of total probability we know that every pdf can be conditionally factorized,
\begin{equation}
    p(\chi)=p(x)\cdot p(s|x)=p(s)\cdot p(x|s),
    \label{eq:factorDist}
\end{equation}
so taking natural logarithm of both sides yields
\begin{equation}
    \log{p(\chi)}=\log{p(x)}+\log{p(s|x)}=\log{p(s)}+\log{p(x|s)},
    \label{eq:logP}
\end{equation}
which is simply a way of describing the joint distribution in terms of marginal and conditional log-likelihoods. Note that since there is a connection between log-likelihood and information, we can also think about
(\ref{eq:logP}) as summing the marginal and conditional information. In the following sections we will use this formulation to describe the original channel filter (CF) \cite{grime_data_1994} and derive new CF variants.   


%\od{Figure \ref{fig:fusionChart} presents the steps taken in the derivation of heterogeneous CF with the assumptions indicated next to each step. The chart is also divided into two parts indicated by the block colors. The exact CF, for homogeneous state vectors is indicated in navy blue. The approximate CF, which is described in the following section is indicated by light blue.}


\subsubsection{Original CF}
We are interested in the estimated underlying distribution of the state $\chi$ given information $Z_i$ and $Z_j$ at agents $i$ and $j$, respectively. Using a distributed variant of Bayes' rule, ref. \cite{chong_distributed_1983} show that the exact posterior pdf conditioned on common information of $i$ and $j$ can be achieved using
\begin{equation}
    p_f(\chi|Z_i\cup Z_j)=\frac{1}{C}\cdot \frac{p_i(\chi|Z_i)p_j(\chi|Z_j)}{p_c(\chi|Z_i\cap Z_j)},
    \label{eq:bayesCF}
\end{equation}
where $C$ is a normalizing constant and $c$ denotes common information. By substituting linear Gaussian distributions ($p(\chi)= \mathcal{N}(\tilde{\chi},\tilde{P}$)), taking logs and differentiating once for the information vector ($\tilde{P}^{-1}_f \tilde{\chi}_f$) and twice for the information matrix ($\tilde{P}^{-1}_f$), \cite{chong_distributed_1983} obtains
the fusion equations,
\begin{equation}
    \begin{split}
        \tilde{P}^{-1}_f&=\tilde{P}^{-1}_i+\tilde{P}^{-1}_j-\tilde{P}^{-1}_c \\
        \tilde{P}^{-1}_f \tilde{\chi}_f=&\tilde{P}^{-1}_i \tilde{\chi}_i+\tilde{P}^{-1}_j \tilde{\chi}_j-\tilde{P}^{-1}_c \tilde{\chi}_c.
    \end{split}
\end{equation}
These equations are in the basis of the CF. In  \cite{grime_data_1994}, Grime and Durrant-Whyte suggest adding a filter on the communication channel (hence CF) between any two agents in a tree network. The CF tracks the common information transferred, thus allowing exact subtraction of common information to avoid double counting. While this operation leads to exact 'locally centralized' fusion for full rate communication, the original CF formulation does not exploit the structure of the estimation problem, and thus communicates w.r.t. the full joint pdf $p(\chi)$, even if agent $i$ only cares about a subset $(x,s_i)$ and $j$ about $(x,s_j)$, as shown in Fig. \ref{fig:fusionChart}. 
This motivates the extension of the CF into a family of heterogeneous fusion methods that utilize the structure of the problem to conditionally factorize subsets of the joint distribution.

%Fig. \ref{fig:fusionChart} show different members of the heterogeneous fusion family...

%\nisarComm{Again, you are presuming that the audience is in your head: don't assume that readers will remember or recognize the full details of the CF -- you should add a few more key facts regarding the need to have a separate filter at each node that tracks the common information in the tree network (i.e. which IS the CF at each node! hence the name...), and connect back to your main argument one level deeper than before: the CF algorithm (while leading to exact `locally centralized' fusion -- something which you did not mention yet, btw!) does not exploit structure of the estimation problem, and thus communicates w.r.t. all of $\chi$, even if node $i$ only cares about $(x,s_i)$ and $j$ about $(x,s_j)$, as shown in Fig. 2 ... this would establish WHY the CF is in particular worthy of theoretical attention, but also again foreshadows the next part to bolster flow of the paper...}


\subsubsection{Factorized CF}
Using factorization we can rephrase: %(\ref{eq:bayesCF}):
\begin{equation}
    \begin{split}
     p_f&(\chi|Z_i\cup Z_j)= \\
     &\frac{1}{C}\cdot\frac{p_i(x|Z_i)p_j(x|Z_j)}{p_c(x|Z_i\cap Z_j)}\cdot\frac{p_i(s|x,Z_i)p_j(s|x,Z_j)}{p_c(s|x,Z_i\cap Z_j)}
     \end{split}
     \label{eq:exactFusion}
\end{equation}
\lemma {1} If a state $s$ is said to be unobservable by agent $j$, the following is implied: $p_j(s|Z_j)=p_j(s)$, thus $p_j(s|x,Z_j)=p_j(s|x)$.\\
From Lemma 1 we can deduce this important conclusion: $p_j(s|x,Z_j)=p_c(s|x,Z_i\cap Z_j)=p_j(s|x)$, in other words, the information available at agent $j$ regarding $s$ equal the common information between $i$ and $j$ and (\ref{eq:exactFusion}) can be written
\begin{equation}
    \begin{split}
     p_f(\chi|Z_i\cup Z_j)= 
     \frac{1}{C}\cdot\frac{p_i(x|Z_i)p_j(x|Z_j)}{p_c(x|Z_i\cap Z_j)}\cdot p_i(s|x,Z_i).
     \end{split}
     \label{eq:exactFusionFinal}
\end{equation}
Another way to look at it is by starting from $p_f(x,s|Z_i\cup Z_j)$, factorizing and claiming $p_f(s|x,Z_i\cup Z_j)=p_i(s|x,Z_i)$ will give us the same result. %\\
Taking natural logarithm of equation (\ref{eq:exactFusionFinal}) and dropping $Z$ for ease of notation, the exact fusion posterior under the assumption that $s$ is independent of $Z_j$ can be written
\begin{equation}
    \begin{split}
    log[p_f(\chi)] &= \log[p_i(x)]+\log[p_j(x)]-\log[p_c(x)]
    \\&+\log[p_i(s|x)]+\tilde{C}(i,j). 
    \end{split}
     \label{eq:logExactFusion}
\end{equation}
This important result implies that if agent $j$ does not gain any information regarding state $s$, it should only send marginal information on state $x$ to agent $i$. We name this derivative ``Factorized CF" (F-CF), since the distribution was factorized into two contributions: 1) marginal information regarding $x$, gathered and shared by the two agents and 2) conditional information regarding $s$ only from agent $i$. The transition from the original CF to the factorized CF is shown in Fig. \ref{fig:fusionChart}, and is enabled under the assumption that a subset of the states is unobservable by one of the agents. This fusion rule provides a possible $\mathbb{F}$ sought in (\ref{eq:probStatement}): here, the communicated distributions are not over the same set of states as $i$ sends $p_i(\chi_i|Z^{-}_{i,k})$ (over $\chi$) and $j$ sends only $p_j(x_{j,k}|Z^{-}_{j,k})$ (over $x$). The posterior fused pdfs, however, are equal in $i$ and $j$.

Now consider the case where the subset $s$ can be divided into two other subsets $s_i$ and $s_j$ ($s=[s_i^T,s_j^T]^T$). So the state vector is $\chi=[x^T,s_i^T,s_j^T]^T$, and $\chi\sim p(\chi)=p(x,s_i,s_j)$. We assume that $s_i$ is not observable by agent $j$ and $s_j$ is not observable by agent $i$, i.e. $s_i\perp Z_j$ and $s_j\perp Z_i$. Similarly to (\ref{eq:exactFusion}) we can factor the different subsets of states:
\begin{equation}
    \begin{split}
     &p_f(\chi|Z_i\cup Z_j)=\frac{1}{C}\cdot\frac{p_i(x|Z_i)p_j(x|Z_j)}{p_c(x|Z_i\cap Z_j)}\cdot \\&\frac{p_i(s_i|x,Z_i)p_j(s_i|x,Z_j)}{p_c(s_i|x,Z_i\cap Z_j)}\cdot\frac{p_i(s_j|x,s_i,Z_i)p_j(s_j|x,s_i,Z_j)}{p_c(s_j|x,s_i,Z_i\cap Z_j)}
    \end{split}
    \label{eq:exactFusion_3states}
\end{equation}


Applying Lemma 1 on the two last expressions, taking the natural logarithm and again dropping $Z$ for notation convenience, we can write the fusion equation as,
\begin{equation}
    \begin{split}
        \log[p_f(\chi)] = \log[p_i(x)]+\log[p_j(x)]-\log[p_c(x)&]\\ 
         +\log[p_i(s_i|x)]+\log[p_j(s_j|x,s_i)]+\tilde{C}(i,j&) 
    \end{split}
     \label{eq:logExactFusion_3states} 
\end{equation}
We assume that the two subsets $s_i$ and $s_j$ are conditionally independent given $x$ ($s_i\perp s_j|x$), then $\log[p_j(s_j|x,s_i)]=\log[p_j(s_j|x)]$ and (\ref{eq:logExactFusion_3states}) becomes
\begin{equation}
    \begin{split}
        \log[p_f(\chi)] &= \log[p_i(x)]+\log[p_j(x)]-\log[p_c(x)] \\
    &+\log[p_i(s_i|x)]+\log[p_j(s_j|x)]+\tilde{C}(i,j).
    \end{split}
     \label{eq:logExactFusion_3states_B}
\end{equation}
 
We name this CF derivative ``Bi-directional factorized CF" (BDF-CF). Here we can see symmetry between the two agents: the agents contribute marginal information regarding the state $x$, and then each agent shares unique conditional information regarding each other's unobservable states $s_i$ and $s_j$. As in the F-CF, this gives another fusion rule $\mathbb{F}$, only now $i$ sends its marginal pdf over ($x,s_i$) and $j$ sends its marginal over ($x,s_j$). The posterior fused pdfs are again equal.
 
It is important to note that the independence assumption ($s_i\perp s_j|x$) is not trivial. To highlight this, Fig. \ref{fig:GraphModel} presents two different Bayesian networks. In (a) the random variables are static, and the assumption holds since $x$ d-separates $s_i$ and $s_j$. On the other hand in (b), some of the variables are dynamic, which is referred to as a partially dynamic Bayesian network \cite{chong_graphical_2004}. Here we can see that in a filtering scenario, the Chapman-Kolmogorov update, which marginalizes over past states, will result in coupling between $s_i$ and $s_j$, and the assumption  no longer holds. In Sec. \ref{sec:DynamicSim}, we describe one solution to this problem. 

The ``Bi-directional factorized CF" is a mathematically equivalent version of the original CF. However, as shown later in \ref{sec:NumExample}, when the above assumptions are met, it enables considerable reduction in communication requirements by sending only new and relevant information. While the BDF-CF has the potential of saving communication costs, it still requires that every agent holds a local version of the full state vector and to communicate information regarding locally unique states. By sacrificing part of the ``exactness" of the CF over less relevant states, we can gain significant reduction in both computation and communication requirements. This brings us to a new family of approximate CF methods. %%developed in the following section.

\subsubsection{Approximate CF}
As we saw in (\ref{eq:logExactFusion_3states_B}), mathematical equivalence to the original CF is achieved under the assumption that $s_j/s_i$ are unobservable by agents $i$ and $j$, respectively, and that that these states are conditionally independent given $x$ requires agent $i$ to send the information regarding $s_i$ (and vice-versa). This might still require considerable communication volume, for example, when $s_i$ are agent $i$'s ownship states for a typical navigation filter, which typically has 15 or more states \cite{dourmashkin_gps-limited_2018}. 

By acknowledging that each agent has a different, but overlapping, subset of states of interest, and does not directly contributes to all its neighbor states of interest, we can reduce it by communicating only the local marginals ($p_i(x) / p_j(x)$). The approximate fusion rule at $i$ is then
\begin{equation}
    \begin{split}
    \log[p_{i,f}(\chi)] &= \log[p_i(x)]+\log[p_j(x)]-\log[p_c(x)]\\
    &+\log[p_i(s_i|x)]+\log[p_i(s_j|x)]+\tilde{C}(i,j), 
    \end{split}
    \label{eq:logApproxFusion_3states_i}
\end{equation}
%%
\begin{comment}
\begin{equation}
    \begin{split}
    \log[p_{j,f}(\chi)] &= \log[p_i(x)]+\log[p_j(x)]-\log[p_c(x)]\\
    &+\log[p_j(s_i|x)]+\log[p_j(s_j|x)]+C(i,j) 
    \end{split}
     \label{eq:logApproxFusion_3states_j}
\end{equation}
\end{comment}
\noindent where equivalent equation can be written for agent $j$ by switching $i$ with $j$ for the conditional pdfs over $(s_i,s_j)$.
The expressions $\log[p_i(s_i|x)]$ and $\log[p_i(s_j|x)]$ represent the local conditional information agents $i$ holds regrading the states not mutually monitored by $i$ and $j$. This conditional information will not be updated in the fusion step, thus resulting an approximation. We name this CF variant ``Approximate BDF-CF". The function formulation for $\mathbb{F}$ still holds here, since this fusion rule will lead to different fused posterior results for agents $i$ and $j$. It is important to note that while the conditional pdfs, $p_i(s_i|x)$ and $p_i(s_j|x)$, are not updated and do not gain information, the local joint pdf $p_i(x,s_i,s_j)$ at each agent do get updated. This is the result of the marginal update for $x$, i.e. each agent `infers' their own global joint updates for local exclusive variables, thus `indirectly' update local variables.

Now we take the next step to derive a heterogeneous state CF (HS-CF). This version relaxes the assumption that all agents across the network hold a local version of the same global state $\chi$, and instead only keep track of locally relevant subsets of states. In our formulation this relates to the local states at $i/j$, such that 
$\chi_i=\begin{bmatrix}x^T,s_i^T\end{bmatrix}^T$ and $\chi_j=\begin{bmatrix}  x^T,s_j^T\end{bmatrix}^T$.
This means that after fusing the marginal information regarding $x$, agents $i$ and $j$ locally update only the relevant conditional information, %%as can be seen in the following equations, 
\begin{equation}
    \begin{split}
    \log[p_{i,f}(\chi_i)] &= \log[p_i(x)]+\log[p_j(x)]-\log[p_c(x)]\\
    &+\log[p_i(s_i|x)]+\tilde{C}(i,j)
     \label{eq:logHeteroFusion_3states_i}
     \end{split}
\end{equation}
\begin{equation}
    \begin{split}
    \log[p_{j,f}(\chi_j)] &= \log[p_i(x)]+\log[p_j(x)]-\log[p_c(x)]\\
    &+\log[p_j(s_j|x)]+\tilde{C}(i,j) 
     \label{eq:logHeteroFusion_3states_j} \\
     \end{split}
\end{equation}
Comparing (\ref{eq:logApproxFusion_3states_i}) to (\ref{eq:logHeteroFusion_3states_i}), we can see the main difference in the fusion of homogeneous and heterogeneous pdfs, respectively, as it translates to the fusion equations. While for the fusion of two homogeneous pdfs, the agents are required to locally update the joint information regarding $s_i$ and $s_j$, in the heterogeneous fusion, each agent only updates locally relevant states. HS-CF fusion gives another fusion rule $\mathbb{F}$ for the problem statement in (\ref{eq:probStatement}). The posterior fusion pdfs are given by (\ref{eq:logHeteroFusion_3states_i})-(\ref{eq:logHeteroFusion_3states_j}) and yield different posteriors at each agent, corresponding to the local heterogeneous joint pdf held by that agent. 

\subsection{Gaussian Distributions}
\subsubsection{Preliminaries}
To derive a closed form fusion rule for the case of linear Gaussian distributions we first need an expression for (\ref{eq:logP}) in information form.
Assume the full joint distribution over the state $\chi$, defined in (\ref{eq:stateDef}), is a multivariate Gaussian with mean $\mu$ and covariance matrix $\Sigma$,
\begin{equation}
    \mu=\begin{bmatrix}
    \mu_x\\
    \mu_s\\
    \end{bmatrix}, \ \ \ \ \ \ \ \Sigma=\covMat  \\
\end{equation}
where $x$ and $s$ denote two correlated subsets of the joint state $\chi$.
The information form of $\chi$ is given by
\begin{equation}
    \zeta=\Sigma^{-1}\mu=\begin{bmatrix}
    \zeta_x\\
    \zeta_s\\
    \end{bmatrix}, \ \ \ \ \ \ \ \Lambda=\Sigma^{-1}=\infoMat  \\
    \label{eq:infoDef}
\end{equation}
The pdf in information form for the normally distributed state $\chi$, with mean $\zeta$ and covariance matrix $\Lambda$ is
\begin{equation}
    p(\chi;\zeta,\Lambda) \propto \exp\bigg({-\frac{1}{2}\zeta^T\Lambda^{-1}\zeta-\frac{1}{2}\chi^T\Lambda \chi+\zeta^T\chi\bigg)}
    \label{eq:infoDist}
\end{equation}
This pdf can also be expressed using factorization (\ref{eq:factorDist}), where the marginal and conditional of a Gaussian are also Gaussian, 
\begin{equation}
    \begin{split}
         p(x)&=\mathcal{N}(x;\bar{\zeta}_x,\bar{\Lambda}_{xx}) \\
         p(s|x)&=\mathcal{N}(s;\zeta_{s|x},\Lambda_{s|x}) 
         \label{eq:pdfDef}
    \end{split}
\end{equation}
where (from \cite{thrun_probabilistic_2005,thrun_graph_2006}) 
 \begin{equation}
     \begin{split}
         \bar{\zeta}_x = \zeta_x-\Lambda_{xs}\Lambda^{-1}_{ss}\zeta_s&, \ \ \ \ \bar{\Lambda}_{xx}=\Lambda_{xx}-\Lambda_{xs}\Lambda^{-1}_{ss}\Lambda_{sx} \\
         \zeta_{s|x} = \zeta_s-\Lambda_{sx}x&, \ \ \ \ \Lambda_{s|x}=\Lambda_{ss}
         \label{eq:marg_cond}
     \end{split}
 \end{equation}
Plugging (\ref{eq:infoDist})-(\ref{eq:marg_cond}) into (\ref{eq:logP}), gathering like terms and separating into first and second order terms gives the information vector $\zeta$ and information matrix $\Lambda$, respectively, 
\begin{equation}
\begin{split}
    &\ln{p(\chi)}\propto\begin{pmatrix} \bar{\zeta}_x+\Lambda_{xs}\Lambda^{-1}_{ss}\zeta_s \\ \zeta_s\end{pmatrix}^T\begin{pmatrix} x \\ s \end{pmatrix}\\
    &-\frac{1}{2}\begin{pmatrix} x \\ s \end{pmatrix}^T
    \begin{pmatrix} \bar{\Lambda}_{xx}+\Lambda_{xs}\Lambda^{-1}_{ss}\Lambda_{sx}  & \Lambda_{xs} \\
    \Lambda_{sx} & \Lambda_{ss}\end{pmatrix}
    \begin{pmatrix} x \\ s \end{pmatrix}\\
    &=\zeta^T\chi-\frac{1}{2}\chi^T\Lambda \chi 
    \end{split}
    \label{eq:lnDerivation}
\end{equation}
From the above equation it is straightforward to see that we can  write the information form of $\chi$ as the sum of two contributions: (i) marginal information ($\bar{\zeta}_x,\bar{\Lambda}_{xx}$) and (ii) contribution from the conditional information 
\begin{equation}
    \begin{split}
        \zeta=\begin{pmatrix} \bar{\zeta}_x \\ 0\end{pmatrix}&+\begin{pmatrix} \Lambda_{xs}\Lambda^{-1}_{ss}\zeta_s \\ \zeta_s\end{pmatrix}\\
        \Lambda=\begin{pmatrix} \bar{\Lambda}_{xx}  & 0 \\
    0 &0\end{pmatrix}&+\begin{pmatrix} \Lambda_{xs}\Lambda^{-1}_{ss}\Lambda_{sx}  & \Lambda_{xs} \\
    \Lambda_{sx} & \Lambda_{ss}\end{pmatrix}
    \end{split}
    \label{eq:localInfFusion}
\end{equation}
%It is interesting to see that in this formulation, the conditional terms, which relate to the unique states remain without change \nisarComm{this statement is a bit vague/confusing -- be more precise by specifying variables being referred to?}.

These expressions formulate the local reassembling of information from a marginal distribution, over \emph{x}, to the joint state information, over $\chi=[x^T,s^T]^T$. It is of interest to develop closed form expressions for fusion of heterogeneous joint pdfs from different agents.
\subsubsection{Fusion}
 Define $\Bar{\zeta}^f_x$ and $\Bar{\Lambda}^f_{xx}$ to be the \emph{fused} marginal information vector and matrix, respectively, of $x$, represented in information form.
Without loss of generality, the fused information can be achieved by using different fusion methods, exact and approximate. In the scope of this work we focus on the CF for exact fusion. Then the fused the marginal information for Gaussian distributions is given by
\begin{equation}
    \begin{split}
        \bar{\zeta}^f_x &= \bar{\zeta}^i_x+\bar{\zeta}^j_x-\bar{\zeta}^c_x \\
        \bar{\Lambda}^f_{xx} &= \bar{\Lambda}^i_{xx}+\bar{\Lambda}^j_{xx}-\bar{\Lambda}^c_{xx}
        \label{eq:GaussMarginal}
    \end{split}
\end{equation}
where $c$ denotes the common information. The HS-CF fusion rule, eqs.  (\ref{eq:logHeteroFusion_3states_i})-(\ref{eq:logHeteroFusion_3states_j}), for Gaussian pdfs is given by the simple closed form expression
\begin{equation}
    \begin{split}
        \zeta^i=\begin{pmatrix} \bar{\zeta}^f_x \\ 0\end{pmatrix}&+\begin{pmatrix} \Lambda^i_{xs}(\Lambda^{i}_{ss})^{-1}\zeta^i_s \\ \zeta^i_s\end{pmatrix}\\
        \Lambda^i=\begin{pmatrix} \bar{\Lambda}^f_{xx}  & 0 \\
    0 &0\end{pmatrix}&+\begin{pmatrix} \Lambda^i_{xs}(\Lambda^i_{ss})^{-1}\Lambda^i_{sx}  & \Lambda^i_{xs} \\
    \Lambda^i_{sx} & \Lambda^i_{ss}\end{pmatrix}
    \label{eq:fusionEq}
    \end{split}
\end{equation}
where $\Bar{\zeta}^f_x$ and $\Bar{\Lambda}^f_{xx}$ are given in (\ref{eq:GaussMarginal}).

An equivalent expression for the fused information at agent $j$ is achieved by switching $i$ with $j$. It is important to note that as we see from (\ref{eq:fusionEq}), the information in the fused marginal will be the same for agents $i$ and $j$, but there is information that is left locally (the right part of the equations) which means that after fusion, the \emph{local joint} information in $i$ (w.r.t. $x$ and $s_i$) and $j$ (w.r.t. $x$ and $s_j$) will be different. We can also see from this expression that while the agents gain only marginal information, the full local joint distribution over the states (inverse of the information) will be updated.

As stated above, we can use various fusion methods to fuse the marginal information, in the scope of this paper we focus on the CF and its derived derivatives. However, to demonstrate how this can be used more generally, we would like to draw special attention to the case of Naive Bayes fusion to prove Lemma 1 in \cite{ahmed_factorized_2016}, which was originally stated without formal proof. Following \cite{ahmed_factorized_2016}, consider the fusion of two Gaussian-distributed independent estimates $p_i(x,s)$ and $p_j(x)$. Using Naive Bayes as the fusion method, the fused marginal information vector and matrix take the form
\begin{equation}
    \begin{split}
        \bar{\zeta}^f_x &= \bar{\zeta}^i_x+\bar{\zeta}^j_x \\
        \bar{\Lambda}^f_{xx} &= \bar{\Lambda}^i_{xx}+\bar{\Lambda}^j_{xx}.
        \label{eq:Lem1proof}
    \end{split}
\end{equation}
Plugging (\ref{eq:Lem1proof}) into (\ref{eq:fusionEq}) and using (\ref{eq:marg_cond}),
\begin{equation}
    \begin{split}
        \zeta^i=\begin{pmatrix} \zeta^i_x \\ \zeta^i_s\end{pmatrix}&+ \begin{pmatrix}\bar{\zeta}^j_x \\ 0\end{pmatrix}\\
        \Lambda^i=\begin{pmatrix} \Lambda^i_{xx}  & \Lambda^i_{xs} \\
    \Lambda^i_{sx} & \Lambda^i_{ss}\end{pmatrix}&+\begin{pmatrix} \bar{\Lambda}^j_{xx}  & 0 \\
    0 &0\end{pmatrix}
    \label{eq:Lemma1Eq}.
    \end{split}
\end{equation}
Transformation back into covariance form thereby proves Lemma 1 in \cite{ahmed_factorized_2016}. 












==> Text/Conservative_Marginalization.tex <==
Principals / comments for conservative marginalization:
\hl{I already addressed conservative filtering in} \ref{subsec:consFiltering}. \hl{Think if there is anything else to say.}
\begin{itemize}
    \item Information (factors) affected by local states should remain conditionally independent given the common states.
    \item Local and common states should not get more information than they ought to due to marginalization.
    \item The approximation should not require more computation / work than the vanilla CF.
    \item A local state shouldn't be affected directly (i.e., get a factor) by another agent's local state.
    \item Should a message after marginalization have 0 information?
    \item What is the bound on the information that is reduced / gained due to marginalization?
\end{itemize}

\textbf{Claim:} An approximate marginalization using a ``smaller" (conditional) information is \emph{not} conservative.

\textbf{Proof:}
The differential entropy of the joint Gaussian distribution $p(x,y)$ is given by (Bishop 1.112):
\begin{equation}
    H[x,y] = H[y|x]+H[x],
    \label{eq:diffEnt}
\end{equation}
where For Gaussian distributions (Bishop 1.110):
\begin{equation}
    H[x] = \frac{1}{2}\{1+\ln(2\pi\sigma_x^2)\},
\end{equation}
and (by induction)
\begin{equation}
    H[y|x] = \frac{1}{2}\{1+\ln(2\pi\sigma_{y|x}^2)\}.
\end{equation}
We can easily see that the entropy increases with the variance.\\
Now, assume $y|x$ is more informative than $\hat{y}|x$, i.e., $\sigma_{y|x}<\sigma_{\hat{y}|x}$, then $H[y|x]<H[\hat{y}|x]$.
Rearranging \ref{eq:diffEnt}:
\begin{equation}
    \begin{split}
        H[x]=H[x,y]-H[y|x]>H[x,y]-H[\hat{y}|x]=H[\hat{x}],
    \end{split}
\end{equation}
where we assumed $H[x,y]$ is constant.\\
Since $H[x]>H[\hat{x}]$, $\sigma_x>\sigma_{\hat{x}}$ the approximation is not conservative.

\od{What is the connection to split-CI?\\ What is the connection to jucntion tree? }

==> Text/FactorAlgorithms.tex <==
In section \ref{sec:factorCF} we derived equations that form the basis of the conditionally factorized CF family of algorithms. In this section use Factor graphs to develop the algorithms for heterogeneous decentralized data fusion. To get insight and be able to track the common information explicitly we first consider linear Gaussian distributions and use the iFactor version of the factor graph. Since assumptions regarding conditional independence requires different treatment in the static vs dynamic cases, we will analyze the static case first.   
\subsection{Static Problems}

We start our analysis before the first measurement and fusion step, and look at the local graph of agent \emph{i}.
There are three main steps performed on the graph, in the brackets we see the local distribution represented by the graph:
\begin{enumerate}
    \item \textbf{Fuse local measurements} = add measurement factors to the graph - $p_i(x,s_i|m_i^1,y_i^1)$.
    \item \textbf{Prepare local message} = add \emph{anti-factor} and refactor graph - $p_i(x,s_i|m_i^1,y_i^1)=p_i(x|m_i^1,y_i^1)\cdot p_i(s_i|x,m_i^1,y_i^1)$.
    \item \textbf{Fuse} = add all received fusion factors to the graph - $p_i(x,s_i|m_i^1,y_i^1,m_j^1,y_j^1)$.
\end{enumerate}
%The term \emph{anti-factor} was introduced in \cite{cunningham_ddf-sam_2013} as a mean to remove information in a graph-SLAM algorithm. Similarly we use it here to account for implicit common information by subtracting it before marginalization.

\od{Add figure that show graphs}

\subsection{Dynamic Problems}
A dynamic fusion problem can be divided into two sub-problems: (i) full time history estimate, i.e. without marginalization of past states in the local estimation step, as common in SLAM problems where robot past pose states are kept (ii) sliding window estimate, where there is a marginalization of past states, as done in Kalman filtering (for a sliding window of 1). As will be shown, in heterogeneous fusion, local marginalization of past states leads to implicit common information not tracked by the channel filter and results double counting. 
We start with analyzing problem (i) and than show the challenge that arise due to marginalization and offer an approximate conservative marginalization step to be able to separate the implicit and explicit common information and avoid double counting.

There are two main technical insights that enable the tracking of common information in a dynamical problems and allow marginalization. First, we look at what happens in the prediction step and how it is translated to the iFactor graph.\\
The augmented state (AS) filter \cite{chong_comparison_2014} estimates the distribution of the joint state $x_{k:n|k}=[x_{k|k}^T,...,x_{n|k}^T]^T$, accumulated over a time window from initial time $t_n$ up to the present time $t_k$. 
The prediction step in ref.\cite{chong_comparison_2014} is given in state space. We present an information space version of it and name it \emph{iAS}.
The predicted information matrix and vector are given by: 
\begin{equation}
    \begin{split}
       \Lambda_{k:n|k-1}&=
       \begin{pmatrix} Q^{-1} & -Q^{-1}\mathbf{F}  \\
       -\mathbf{F}^TQ^{-1}  & \Lambda_{k-1:n|k-1}+\mathbf{F}^TQ^{-1}\mathbf{F}
        \end{pmatrix},\\
       \zeta_{k:n|k-1}&=
       \begin{pmatrix}Q^{-1}Gu_k \\ 
       \zeta_{k-1:n|k-1}-\mathbf{F}^TQ^{-1}Gu_k\end{pmatrix},
   \end{split}
    \label{eq:iAS_pred_Final}
\end{equation}
where $\mathbf{F}=\big[F_{k-1} \ \ 0_{m \times m(k-n-2)} \big ]$ and $m$ is the size of the (not augmented) state vector. \\
The main insight from (\ref{eq:iAS_pred_Final}) is that the predicted state information block $\Lambda_{k|k-1}=Q^{-1}$ (left upper block in $\Lambda_{k:n|k-1}$) does not have terms relating past information states (and similarly in the information vector), i.e. it can be separated in an additive manner. The predicted information matrix can be expressed as a summary of three factors: 
\begin{equation}
    \begin{split}
       \Lambda_{k:n|k-1}&=\overbrace{
       \begin{pmatrix} Q^{-1} & 0  \\
       0  & 0
        \end{pmatrix}}^{f(x_k)}
        +\overbrace{\begin{pmatrix} 0 & -Q^{-1}\mathbf{F}  \\
       -\mathbf{F}^TQ^{-1}  & 0
        \end{pmatrix}}^{f(x_k|x_{k-1}:n)}\\
        &+\underbrace{\begin{pmatrix}0 & 0  \\
       0 & \Lambda_{k-1:n|k-1}+\mathbf{F}^TQ^{-1}\mathbf{F}
        \end{pmatrix}}_{f(x_{k-1}:n)},
    \end{split}
    \label{eq:iAS_pred_Final}
\end{equation}
where here we omit the information vector from the factor notation for abbreviation.
\od{need to reference a graph}\\
As will be demonstrated, in order to be able to track common information, 
it is of interest to perform approximate conservative marginalization. We first state fact $10.11.18$ from \cite{bernstein_scalar_2018} about two positive-definite (PD) matrices $A,B$:
\begin{equation}
    (A+B)^{-1}\leq \frac{1}{4}(A^{-1}+B^{-1}),
    \label{eq:inverseInequality}
\end{equation} 
where equality holds when $A=B$.  
For a series of PD matrices $A_1...A_n$ we can recursively use eq. (\ref{eq:inverseInequality}) to get:
\begin{equation}
    (A_1+A_2+...+A_n)^{-1}\leq \sum_{i=1}^{n}\frac{1}{4^i}A_i^{-1}
    \label{eq:inverseInequality}
\end{equation} 
The second insight then results from this equation, where a marginalization of a past variable requires taking the inverse of two kind of factors connected to this variable, local factor and common factor. The local factor includes implicit common information that is not tracked by the channel filter and will be coupled to the common factor by taking the inverse. Using this approximation we are able to keep the two factors separated in a conservative way.\\



==> Text/Numerical_example.tex <==

To highlight the potential gain in communication and computation complexity of the proposed CF$^2$ methods, consider a numerical example for the problem of tracking 11 stationary ground targets by 10 agents (trackers), where each agent computes a local KF estimate. Each agent $i$ has 6 unknown ownship position states $s_i$ and takes measurements to $n_i$ targets, each has 2 position states $x_t$ (East,North). The full state vector then has 82 states. Assume tree topology in ascending order, where 7 agents take measurements to 2 targets and agents 2, 6 and 10 take measurements to 3 targets, such that each agent has 1-2 targets in common with its neighbors. Now, using the same logic as before, assume that each agent is only concerned with the target it takes measurements to and its ownship position states. Each agent then has a local state vector of only 10-12 states for tracking 2-3 targets, respectively. 

Table \ref{tab:table2} presents a comparison between the different channel filters, where the baseline is the original CF, with each agent estimating the full 82 states vector. For the communication data requirement we assume 'double' precision (8 bytes per element), where the matrices are covariance matrices, thus only need to communicate upper diagonal ($n(n+1)/2$ elements). Each agent computation complexity is determined by the cost of inverting an $n\times n$ matrix, with $n$ as the number of states. We can see from the table that while the exact BDF-CF offers about 66.5\% reduction in communication, the approximate methods saves about 99.8\% in communication. The main advantage of the HS-CF then is in  computation, since each agent only estimates the locally relevant states, i.e. it scales with subset of states and not with number of agents and targets.  



\begin{table}[t]
\caption{Data communication requirements and computational complexity for different fusion methods}
%\label{table_example}
\begin{center}
\begin{tabular}{c c c c}
  {\bf Method} & {\bf Data [bytes]  }& {\bf Data [\%CF]  }  & {\bf Complexity}\\ 
\hline
  {CF}   & 501840     & ---  & $O(82^3)$  \\
\hline
  {BDF-CF}   & 168168     & 33.5  & $O(82^3)$  \\
\hline
  {Approximate BDF-CF}   & 1152     & 0.23  & $O(82^3)$  \\
\hline
  {HS-CF}   & 1152     & 0.23  & $O(12^3)$  \\
\end{tabular}
\end{center}
\label{tab:table2}
\vspace{-0.25in}
\end{table}



==> Text/Some_Ideas.tex <==
\begin{itemize}
    \item \textbf{Goal:} The Goal of this work is to explore the applicability and robustness of the FG-DDF framework for the linear case - i.e. \emph{why should you care or want to use this framework}. It will build on and extend \cite{dagan_factor_2021}, \cite{dagan_conservative_2022} which developed the FG-DDF framework and the conservative filtering approach, respectively. 
    \hl{It has to answer the question of why is it better than state of the art? namely DDF-SAM 2.0 }
    
    \item \textbf{Take-home points:}
    \begin{itemize}
        \item We developed a \underline{heterogeneous} DDF framework which is:
        \begin{enumerate}
            \item Conservative
            \item Scalable 
            \item Robust
            \item Applicable: can represent a variety of applications (relevant even for the linear/Gaussian case) 
        \end{enumerate}
    \end{itemize}
    
    %The goal of this work is to empirically explore the nonlinear heterogeneous DDF filtering problem and surface gaps.
    \item \textbf{Application}: 
    To show scalability: Target tracking with multiple agents and target (i.e. large state vector)\\
    To show applicability: Search 
    Height map; occupancy grids; search as in the conditionally factorized paper \cite{ahmed_conditionally_2014}.
    
    \item \textbf{Possible avenues to explore:} 
    \begin{itemize}
        \item Applicability: Showing how it is applicable for different applications, i.e. not just regular KF; CI comparison; cyclic graphs; different architecture - maybe where we have groups of a-cyclic topologies doing CF, but connected to other groups via CI?
        \item Robustness: Message dropout; Time delays; Different models \item Comments from IROS: 
        \begin{enumerate}
            \item The authors stated that channel filter is required to
            guarantee that data is not over-discounted and channel filter requires full rate communication. Full rate communication is sometimes hard to satisfy in some scenarios. How would the proposed method work if full rate communication is not satisfied?
            \item The method requires the prior information of the common variables between each robot. How could it be satisfied in a real-world problem? How would deal with problems such as data association, etc?
            \item The AE would like to add that the paper can be more strengthen with experiments for one or more applications. The authors claimed that the proposed method is rather general but not application-specific. However, the experiment for the tracking task seems to be insufficient to show the generality.
        \end{enumerate}
    \end{itemize}
    
    \item \textbf{Need to do:}
    \begin{itemize}
        %\item Implement IMM
        % \item Implement CI
        \item Develop theory for cyclic networks
    \end{itemize}
    
    
    
    
\end{itemize}





% \graphicspath{{./Figures/}}
% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.48\textwidth]{placeholder.png}
%     \caption{Figure 1 is an illustration of the FG-DDF framework - similar to the fusion paper }
%     \label{fig:fig1}
% \end{figure}



% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.48\textwidth]{placeholder.png}
%     \caption{Figure 2 is a factor graph operations figure }
%     \label{fig:fig2}
% \end{figure}


% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.48\textwidth]{placeholder.png}
%     \caption{Figure 3 is conservative filtering }
%     \label{fig:fig3}
% \end{figure}

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.48\textwidth]{placeholder.png}
%     \caption{Figure 4 is part of the experimental work showing results of the robustness and CI comparison  }
%     \label{fig:fig4}
% \end{figure}

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.48\textwidth]{placeholder.png}
%     \caption{Figure 5 is part of the experimental work showing the IMM/switching model representation  }
%     \label{fig:fig5}
% \end{figure}

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.48\textwidth]{placeholder.png}
%     \caption{Figure 6 is part of the experimental work showing results of the IMM/switching model experiments  }
%     \label{fig:fig6}
% \end{figure}

==> Text/Theory.tex <==
\hl{Decide if this part is required. Another option is to move it to appendix}

In this chapter we want to compare to Paskin's junction tree algorithm and Julier \& Uhlmann's split-CI.

\subsection{Junction Tree}
Here we want to claim that in a static system, if states are `well distributed' between robots, we assume full rate communication and let messages propagate tree width, then the FG-DDF framework with the HS-CF algorithm is equivalent to the distributed junction tree algorithm suggested by Paskin \emph{et al.} \cite{paskin_robust_2004}, \cite{paskin_robust_2005}.

Using the same terminology and definitions ad in \cite{dagan_factor_2021}, a robots' variables would be a clique in the junction tree and the common variables between two robots would be the separation clique.
It can be shown then \od{(show!)} that the messages between robots are equivalent to the message passing algorithm given in \cite{paskin_robust_2004}.

\od{In this part I need to show graphics that emphasize the relation between the two methods and math that shows the equivalence to the message passing algorithm. }


\subsection{Split-CI}
The connection between the HS-CF algorithm and split-CI \cite{julier_general_2009} is still TBD. 
But I have a filling that there is a connection between them. Specifically it seems like the HS-CF can be both a specific case and a generalization of the split-CI. Specific case - when we are talking about different (non-overlapping) parts of the state vector. Generalization - when these parts don't have to be independent, and it is enough for them to be \textbf{conditionally} independent. 

\subsubsection{PDF Interpretation}
First we like to explore what is the pdf interpretation of the split-CI fusion rule would be if the fused pdfs are Gaussian. Starting from the split-CI assumptions: $a=a_d+a_i$ and $b=b_d+b_i$ where the errors associated with $a_d$ and $b_d$ are correlated (dependent) to an unknown degree and the errors associated with $a_i$ and $b_i$ are completely independent from all others. We wish to form a fusion rule that exploits the known degree of independence while accounting for the unknown degree of correlation between the two pdfs.\\
\begin{equation}
    p_f=p_{\omega}(a)p_{1-\omega}(b).
    \label{eq:wepSplitCI}
\end{equation}
If we define the local pdfs as,
\begin{equation}
    \begin{split}
        &p_{\omega}(a)\propto e^{-(x-a)^T(\frac{1}{\omega}A_d+A_i)^{-1}(x-a)/2}\\
        &p_{1-\omega}(b)\propto e^{-(x-b)^T(\frac{1}{1-\omega}B_d+B_i)^{-1}(x-b)/2},
    \end{split}
    \label{eq:WEP_pdfs}
\end{equation}
then the fusion rule given in (\ref{eq:wepSplitCI}) results in the split-CI equations. Where the fused pdf $p_f$ has the following covariance $C$ and mean $c$:
\begin{equation}
    \begin{split}
        &C=\Big [ (\frac{1}{\omega}A_d+A_i)^{-1}+(\frac{1}{1-\omega}B_d+B_i)^{-1}\Big ]^{-1}\\
        &c=C\Big [ (\frac{1}{\omega}A_d+A_i)^{-1}a+(\frac{1}{1-\omega}B_d+B_i)^{-1}b\Big ]
    \end{split}
    \label{eq:splitCI}
\end{equation}

Notice the difference between the covariance terms in (\ref{eq:WEP_pdfs}) and the fused covariance in (\ref{eq:splitCI}); in (\ref{eq:WEP_pdfs}) the covariance $A$ ($B$) is split to a correlated and independent parts, while in (\ref{eq:splitCI}) the two estimates are \emph{fused}, so the information matrices are summed. 

To summarize, in split-CI the independence is in the errors (in the data?) while in the heterogeneous DDF framework the (conditional) independence is of the variables (states).

==> Text/random_thoughts.tex <==



\od{Existing work either solves a smoothing problem \cite{cunningham_ddf-sam_2013}, a static problem \cite{paskin_robust_2004}. In cooperative localization, they either augment the state or ``decorrelate" agents in an ad-hoc manner. While these methods work they might be over-conservative as not all dependencies have to be broken. A deeper understanding of the origin of the dependencies might tell us why these methods work and maybe more importantly when they might break.

Indelman \cite{indelman_graph-based_2012}\cite{indelman_graph-based_2011} - computes dependencies on demand.

Also, check the works of Stergios I. Roumeliotis.}


In \cite{ling_six_nodate} they use CF to send only the map in a SLAM problem.

From Nisar:
A tangentially related thought that only occurred to me just now as I was reading the motivation/background parts talking about covariance intersection:  it would be interesting to compare the results of the heterogeneous CF to something more conventionally used for heterogeneous CF like CI/WEP or inverse CI fusion to see how conservative the estimates become in an undirected acyclic topology, i.e. what gets thrown away or ignored in the wash of doing something like CI to ensure conservativeness. I don't think this is needed for this paper, per se, but a side by side comparison of approaches as part of future work and evaluation could be interesting and insightful.




